Spatial Voice Conversion: Voice Conversion Preserving Spatial Information and Non-target Signals

This paper proposes a new task called spatial voice conversion, which aims to convert a target voice while preserving spatial information and non-target signals. Traditional voice conversion methods focus on single-channel waveforms, ignoring the stereo listening experience inherent in human hearing. Our baseline approach addresses this gap by integrating blind source separation (BSS), voice conversion (VC), and spatial mixing to handle multi-channel waveforms. Through experimental evaluations, we organize and identify the key challenges inherent in this task, such as maintaining audio quality and accurately preserving spatial information. Our results highlight the fundamental difficulties in balancing these aspects, providing a benchmark for future research in spatial voice conversion. The proposed method's code is publicly available to encourage further exploration in this domain.

==> table/similarity.tex <==
\begin{table}[t]
\caption{
    MOS and standard deviation on similarity of synthesized speech between each method and ``\ideal.''
}
\label{table:similarity}
\begin{comment}
bunri 1.9921875 0.9560342383219076
steering 3.4052044609665426 0.9182833381101563
proposed 2.6790123456790123 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Left
bunri 4.141666666666667 0.8971792215357841
steering 3.9745762711864407 0.9782539305606098
proposed 3.007575757575758 0.9730941911587235
ground 4.061538461538461 0.900887136735837
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Right
bunri 1.3880597014925373 0.621870646447751
steering 3.1322314049586777 1.0360617483778394
ground 4.1015625 0.8645794113866869
proposed 2.1025641025641026 0.696568087549032
\end{comment}
\centering \footnotesize
\begin{tabular}{c||c|c|c}
Methods & Stereo & Left & Right \\ \midrule
\inverse &  $ 2.460 \pm 1.235 $ &  $ 3.636 \pm 0.989 $ &  $ 2.348 \pm 1.088 $ \\
\steering &  $ 3.308 \pm 1.058 $ &  $ 3.434 \pm 0.978 $ &  $ 3.282 \pm 1.047 $ \\
\proposed &  $ 2.928 \pm 1.140 $ &  $ 3.633 \pm 1.016 $ &  $ 2.742 \pm 1.015 $ 
\end{tabular}
\vspace{-2mm}
\end{table}


